Fed2: Feature-Aligned Federated Learning

Federated learning learns from scattered data by fusing collaborative models from local nodes. However, the conventional coordinate-based model averaging by FedAvg ignored the random information encoded per parameter and may suffer from structural feature misalignment. In this work, we propose Fed2, a feature-aligned federated learning framework to resolve this issue by establishing a firm structure-feature alignment across the collaborative models. Fed2 is composed of two major designs: First, we design a feature-oriented model structure adaptation method to ensure explicit feature allocation in different neural network structures. Applying the structure adaptation to collaborative models, matchable structures with similar feature information can be initialized at the very early training stage. During the federated learning process, we then propose a feature paired averaging scheme to guarantee aligned feature distribution and maintain no feature fusion conflicts under either IID or non-IID scenarios. Eventually, Fed2 could effectively enhance the federated learning convergence performance under extensive homo- and heterogeneous settings, providing excellent convergence speed, accuracy, and computation/communication efficiency.

==> _txt/.git/objects/5b/39f59fc5ec2660d10feb0d0d072026a9a4851a <==
x•Ž]
Â0"}Î)ö–$M"'â|ñuI·6Ø6%Ý o®àÓÀ0ß̸0MžA+³ãH­¦ºC‹ˆ¶Óe՛¾©´µ(©–Æ'Bí4¶M#0ñ"Ü=Î84ÃaóŸÁotzLèÇ…éªjs¸µ¥…½4RŠìæ=¦ÿI¡V†KĞá×ôNsÖûq"WˆOŸo"\r÷Ê19N'
ñ™iFé

==> _txt/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Federated Learning (FL) have drawn great attention with its great collaborative training performance and data privacy protection benefits~\cite{fl}. 
	In the common setting, FL conducts collaborative training across distributed local models with a homogeneous structure by Federated Averaging (FedAvg) algorithm~\cite{fedavg}, i.e., averaging weights based on their coordinates. 
	However, FedAvg algorithm often suffers from non-negligible accuracy drop when learning rate is not well tuned or the data distributions are highly non-iid~\cite{niid}. 

Previous hypotheses are that the performance drop of FedAvg is mainly caused by averaging diverged parameters, which is called parameter divergence~\cite{niid}. 
	Following that, recent works further showed the parameter divergence is one consequence of the permutation-invariance of neural networks~\cite{fedma}. 
	 That is, two homogeneous models can have different feature encoding ordering in the structure. 
	 Without considering the encoded feature sequences, the coordinate-wise weight averaging could lost learned information and thus hurt the convergence performance~\cite{fedma}. 

To solve this problem, there are several different works proposing matching-based federated averaging algorithms, such as Representation Matching~\cite{representation}, Bayesian Matching~\cite{PFNM}, FedMA~\cite{fedma}, etc. 
	Most of these methods conform to the similar basic process: After certain local training, they re-permute/match the indexes of trained weights based on certain similarity metrics so that similar learned features could be averaged together.
%
Although achieving better performance than coordinate-wise averaging, such post-training matching algorithms have certain limitations:

	(1)	The non-interpretable matching metrics cannot accurately reflect the similarity of encoded features. Most matching metrics usually evaluated the weight similarity of feature similarity by MSE loss to match the averaging units, while small MSE loss doesn’t necessarily indicate similar features; 

	(2)	Most matching algorithms often assume different local models have mostly matchable units. While when facing data heterogeneity, especially highly-skewed non-iid data, different local models can carry distinct features and a forced matching can cause catastrophic information loss;

	(3)	The post-matching algorithm incurs heavy extra communication overhead due to uploading weight/feature for similarity calculation. Besides, using feature-based matching metrics can further require sharing private data to get the features, which compromises the data privacy. 

\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=5.6in]{motivation}
	\vspace{-5mm}
	\caption{The feature encoding comparison between FedAvg and our proposed framework. 
		As the feature indicator, the color of each neuron is determined by its top response class, as defined in Eq.~\ref{eq:2}. 
		The original FedAvg can suffer from feature averaging conflicts due to its chaotic feature encoding among different nodes. 
		In contrast, our framework enables structurally-aligned feature encoding among nodes and reduces such averaging conflicts in both iid and non-iid cases.
		Experiments are conducted on CIFAR10 with 10 collaborative nodes. IID: Each node has data of 10 classes. Non-IID: Each node has data of 5 classes.}
	\label{fig:motivation}
	\vspace{-4mm}
	\end{center}
\end{figure*}


To tackle these limitations, we design a pre-training feature encoding regulation to enforce model's feature allocation.
	Specifically, we construct convolution groups and connect them with different task logits in order to learn the specified feature, i.e., feature allocation. 
	As shown in Fig.~\ref{fig:motivation}, with the feature allocated regulation, our model's feature encoding can conform to the structural form while the natural training often randomly encoded features in the model structure.
	Then along with the feature encoding regulation, we further conduct matched weight averaging within sharing-feature convolutional groups, thus achieving precise feature-matched averaging.

We conduct extensive experiments on general datasets (CIFAR10, 100) with two model structures (VGG, MobileNet).  
	The results demonstrate that our method shows both better convergence accuracy (xx\%-xx\%) and speed (xx\%-xx\%), outperforming previous state-of-the-art works by large margins.
	Especially within the highly-skewed non-iid data distribution, our method still demonstrates robust and effective matching to facilitate the convergence while most previous matching methods cannot. 

==> _txt/6_exp_weishan.tex <==
\vspace{-1.5mm}
\section{Experiment}



\vspace{-1.5mm}
\subsection{\textbf{Experiment Setup}}
\vspace{-1.5mm}
We evaluated the proposed CEL method under simulated data non-iid settings in PyTorch~\cite{?}. 
We assume that all the clients will participate in the model averaging process.
The CNN models we used includes VGG9, VGG16 ~\cite{Simo:2014:arXiv} and MobileNetV1~\cite{?} while the datasets we processed are CIFAR10 and CIFAR100 ~\cite{krizhevsky2009CIFAR}.
For CIFAR10 and CIFAR100 dataset, we use data augmentation (random crops and flips) and normalization processes.

We evaluated the performance margin of our framework versus the baseline, FedAvg, and a state-of-the-art heterogeniety-resistant method, FedMA.  
In this part, the \textit{$\Psi$-Net} structures were kept constant for each CNN model, e.g. we decouple the last two convolutional layers of VGG9, the last 6 convolutional layers for VGG16 and MobileNetV1 and we choose the group size as 10 classes for one-to-many convolutional group mapping in training CIFAR100. 
For the first step, we compared our method and the baseline in comprehensive data non-iid settings.
In each trial, the global training data for each task is divided into several balanced portions, which are allocated to different nodes.

In the Non-iid Spectrum section (Table~\ref{?}) we tested the resistance to distributions with skewed local tasks.
In the Node Scalability part (Table~\ref{?}) where the number of local tasks is constant, we analyzed the feasibility to work with massive nodes and minor local data.  
We also evaluated the convergence speed in the non-iid spectrum of VGG16 on CIFAR100 and provided the results in Fig ~\ref{?}.

To compete with FedMA, we implemented our framework in the Dirichlet non-iid data partitioning condition used by the authors of~\cite{?}.
Meanwhile, we tested the sensitivity of our framework to the number of local training epochs and analyzed its impact to local training effort. 


Finally, to get insights about our \textit{$\Psi$-Net} structural configurations, we studied the impact of two major hyper-parameters, Grouping Depth and Path Granularity.
For Grouping depth sensitivity, we jointly analyzed the testing accuracy of decoupling depthes and activation divergence of diferent layers.
For path granularity, we evaluated the trade-off between fine-grained convolutional groups and model capacity loss caused in decoupling.


% To analyze the performance margin of our method versus the baseline, FedAvg~\cite{?}, we implemented our framework to a variety of FL settings with Non-iid data and tasks. 
% For the first
% SOTA, Acc, local effort, effort,  

% Granularity,
% Grouping depth, Activation divergence
% We use two common convolutional neural networks (CNNs) for evaluation: AlexNet~\cite{Kriz:2012:NIPS} and VGG16~\cite{Simo:2014:arXiv}.
% Two image classification dataset CIFAR10, CIFAR100~\cite{krizhevsky2009CIFAR} are evaluated to demonstrate the generality of our proposed decentralized system.
 
	
\begin{table}[]
\parbox{.49\linewidth}{
\caption{Non-iid Spectrum (CIFAR10).}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{cccccc}
\toprule
                           & N * C & 10x3 & 10x4 & 10x5 & 10x10 \\ \midrule
\multirow{2}{*}{VGG9}      & FedAvg         & 82\% & 84\% & 85\% & 88\%  \\ 
                           & Ours           & 83\% & 88\% & 88\% & 90\%  \\ \midrule
\multirow{2}{*}{MbNet}   & FedAvg         & 67\% & 71\% & 79\% & 85\%  \\ 
                           & Ours           & 86\% & 88\% & 90\% & 91\%  \\ \bottomrule
\end{tabular}}}
\hfill
\parbox{.49\linewidth}{
\caption{Node Scalability (CIFAR10).}
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{cccccc}
\toprule
                           & N * C & 10x5 & 20x5 & 50x5 & 100x5 \\ \midrule
\multirow{2}{*}{VGG9}      & FedAvg         & 85\% & 86\% & 83\% & 83\%  \\
                           & Ours           & 88\% & 88\% & 86\% & 87\%  \\ \midrule
\multirow{2}{*}{MbNet} 	   & FedAvg         & 79\% & 85\% & 81\% & 78\%   \\
                           & Ours           & 90\% & 90\% & 89\% & 88\%   \\ \bottomrule
\end{tabular}}}

\end{table}


\begin{figure*}[]
\centering
\vspace{-3mm}
\includegraphics[width=5.5in]{conv_speed}
\vspace{-5mm}
\caption{Convergence Speed Comparison between FedAvg and Proposed Method (\textbf{CIFAR100}).}
\label{fig:conv_speed}
\vspace{-5mm}
\end{figure*}

\begin{figure*}[]
\centering
\vspace{-3mm}
\includegraphics[width=5.5in]{epoch_efforts}
\vspace{-5mm}
\caption{Local Epoch Influence Evaluation and Training Overhead Comparison with SOTA.}
\label{fig:local_epoch}
\vspace{-5mm}
\end{figure*}


\begin{figure}[]
\centering
\captionlistentry[table]{}
\captionsetup{labelformat=andtable}
\caption{Grouping Depth Sensitivity. \textbf{Left:} Total Variance of each layer. \textbf{Right:} Performance under different grouping depth, showing the grouped models' performance is robust to depth selection in a large range.}
\parbox{.32\linewidth}{
% \begin{figure}[]
\includegraphics[width=1.8in]{4_gradient}
\label{fig:depth}
% \end{center}
}
\qquad
\parbox{.6\linewidth}{
\centering
\vspace{-4mm}
\renewcommand\arraystretch{1.2}
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{c|cccccc|c}
\toprule
VGG16      & C1-2 & C2-2 & C3-2 & C4-2  & C5-2  & FC  & None \\ \midrule
CIFAR10  & 82\%    & 87\%    & \textbf{89\%}  & \textbf{90\%} & \textbf{89\%}          & 87\% & 86\%     \\ \hline
CIFAR100 & 53\%    & 62\%    & 67\%  & \textbf{68\%}   & \textbf{69\%} & \textbf{68\%} & 65\%    \\ \bottomrule
\end{tabular}}}
\vspace{-5mm}
\end{figure}


\begin{figure}[]
\centering
\vspace{-2mm}
\includegraphics[width=2.5in]{granularity}
\vspace{-2mm}
\caption{Path Granularity: one-to-one and one-to-many mapping.}
\label{fig:path}
\vspace{-5mm}
\end{figure}

==> _txt/6_topology.tex <==
\section{\textbf{Distributed Community Structure}}
The choice of communication topology can greatly affect the performance of our learning system. To compromise between training accuracy and communication consumption, we discussed the property of the classic Ring topology~\cite{x,x}, Mesh topology ~\cite{x,lee2006emerging} and the general connected Mesh topology we implemented. 

In this section, we discuss the influence of network topologies to our decentralized collaboration system. 

\subsection{\textbf{Topology Definition}}

\begin{figure}[t]
\begin{center}
	\includegraphics[width=3.3in]{3_topology}
	\caption{Shuffled Decentralized Communication Topology.}
	\label{fig:topology}
	\vspace{-8mm}
\end{center}
\end{figure}

Formally, one network topology can be described with an undirected graph $(V, E)$ where $V$ denotes vertex, \textit{i.e.}, the set of $n$ participating nodes ($V := \{1, 2, \dots, n\}$), and $E$ denotes all the edges in the graph. 
	As in standard representation, we use the adjacent matrix $W \in \mathbb{R}^{n\times n}$ to represent the graph $(V, E)$.
	Also, the adjacent matrix is weighted since each node pair $(i, j)$ can have varied amount of shared parameters, and thus the communication overhead of edge $E(i,~j)$ is also different.
	Therefore, we use the value of each entry $W_{i,j}$ to describe how much communication resource node $i$ and $j$ need for mutual collaboration.

\vspace{-3mm}
\paragraph{\textbf{Ring and Mesh Topology}}
Based on the above definition, the Ring and Mesh topologies could be represented as symmetric matrices where 0 denotes no graph edges in node $i$ and $j$ and $C_{i,j}$ denotes nodes have edges and the communication overhead is $C_{i,j}$.

% \small
\scriptsize
\begin{equation}
\label{eq:adjm}
\begin{split}
	W_{Ring} = \left\{
	\begin{aligned}
		 C_{i,j}, &~~~~\text{If} ~~|i-j| = 1;\\
		 0, &~~~~\text{Otherwise}.
	\end{aligned}
	\right. \hspace{0.1cm} 
		W_{Mesh} = \left\{
	\begin{aligned}
		 C_{i,j}, &~~~~\text{If} ~~i \neq j;\\
		 0, &~~~~\text{Otherwise}.
	\end{aligned}
	\right.
\end{split}
\end{equation}
\normalsize
As we can see from Figure.~\ref{fig:topology}, networks with Ring topology has the least communication edges while Mesh network has the most. Therefore, for the communication resource consumption, the Ring topology brings the least communication overhead and vice versa for Mesh.

\vspace{-3mm}
\paragraph{\textbf{Our Implemented Topology}}
To reach a better parameter consensus in our training, we expect to implement a more interconnected system while keeping the communication load affordable. 
Instead of Ring or Mesh, we implemented a general connected ``Mesh" topology, instead.
The structure of "Mesh" topology in our implementation, on the other hand, is different from the conventional Mesh. 
Actually the complexity of it is between Ring and Mesh topology.
To control the communicational complexity of our topology, we set a hyper parameter $R$ to control the overall number of times that the global dataset is repeated across the whole learning system.
The tasks for each node is randomly and unrepeatedly drawn without replacement from the training data library which contains $R$ replicas of training data for each task.

\subsection{Communication Modeling}
We implemented the Ring and our general connected Mesh topology in the experiments.


To compare our communication cost with that of Federated Learning, the communication cost of our collaborative learning system is measured by the amount of data downloaded by each single node following a point-to-point protocol.  
For centralized learning systems, the communication cost for our system can be formulated as:
\vspace{-1.5mm}
\begin{small}
\begin{equation}
\scriptsize
	\medmuskip=-1mu
	\begin{aligned}
	  Q = \sum_{i=1}^{L-D} B_w f_{i+1} (k_i)^{2} + P\sum_{i=D}^{L} B_w f_{i+1}F_{r}(k_i)^{2} 
	\end{aligned}
	\label{eq:comcent}
\vspace{-0.5mm}
\end{equation}
\end{small}
where $L$ denotes the total number of convolutional layers of our DNN model; $D$ denotes the number of decoupled layers; $B_w$ denotes precision of model weights; $k_i$ denotes kernel width; $P$ denotes the number of functionality structures on each node; $f_i$ denotes the number of input channels of each filter in the $i^{th}$ convolutional layer while $f_{i+1}$ equals to the number of filters in the $i^{th}$ layer; $F_r$ denotes prunning ratio of decoupled layers.

For our learning systems with our ``Mesh" topology, our communication cost can be formulated as:
\vspace{-1.5mm}
\begin{small}
\begin{equation}
\scriptsize
	\medmuskip=-1mu
	\begin{aligned}
	 Q =  N\sum_{i=1}^{L-D} B_w f_{i+1} (k_i)^{2} + P(R-1)\sum_{i=D}^{L} B_w f_{i+1}F_{r}(k_i)^{2} 
	\end{aligned}
	\label{eq:commesh}
\vspace{-0.5mm}
\end{equation}
\end{small}
where $R$ denotes the number of times each task is repeated across the learning system.
From the formulation of communication consumption, we can find that
% For more general cases where the global dataset is repeated several times across the network, the Mesh topology gets more interesting.
% Suppose that training data for task $T_l$ is allocated to $n_l$ nodes. 
% The modules trained for $T_i$ in each node will pick up knowledge about all the other local tasks and a better generalization for this task can be realized through the collaboration of these $n_l$ nodes.
% Similarly, local module for every task can be generalized through the 
% Suppose that the global dataset contains $C$ classes and is repeated $K$ times across the system, the average number of tasks per node turns $\frac{CK}{n}$.

%(i) $W_{i,i}\in (0,1], \forall i \in \{ 1, \dots, n \}$ 
%(i) Only diagonal entries, $W_{ii}, i \in [1,n]$, are necessarily positive. 
%(ii) $W_{i,j}\in [0,1), \forall j \neq i $ while $\sum_j{W_{i,j}} = 1, \forall i \in \{ 1, \dots, n \}$ 
%Meanwhile, the categories of training data allocated to each node will be balanced  
%Each local node can exchange parameters with any other nodes as long as they share training tasks and the data for  which will try to share tasks with as many nodes as possible. 
%That is to say, the replicas of the training data for each specific task are allocated to as many nodes as possible.
%This setting gets more interesting when the overlap ratio get large, which means that each task 
% After each local SGD section, every node will 
% This can be simulated by a random allocation of training data that

% Doesn't limit the overlap ratio of global dataset.
% Better generalization property on average.
% Communication overhead.

% \subsection{\textbf{Communication Formulation}}
% where $C_{i, j}$ denotes the parameter communication requirements between node pair $(i, j)$. 
% %

% In Ring topology, only adjacent nodes need to exchange parameters so the communication matrix is fairly sparse with only two non-zero elements in each row.  
% 	Thus, one clear advantage of Ring topology is the \textit{high communication efficiency}.
% 	However, such low communication overhead also brings a major problem, which is the \textit{limited global consensus}. 
% 	The reason lies in that sparse parameter sharing.
% 	Take Fig.~\ref{fig:topology} as an example, if we denote different color as different task modules, we can see that every single task module is only shared by two neighboring nodes.
% 	When the value of $n$ is large, the task sets on distant nodes become highly divergent, which cause the limited consensus performance of Ring topology. 
% This problem roots in Ring's sparse communication edges and thus can be addressed by other network topologies. 
% 	As a typical example, Mesh topology will be discussed in the next section.
% Regional data trained on local pairs become unbalanced. 
% Besides, the overlap ratio of the global dataset is also limited in ring topology. 
% Since the training data for one single task can only be placed at no more than two nodes, systems with ring topology can maintain two copies of global training dataset at most. 
% Considering that the module for each single task is only collaboratively trained by two nodes, having fewer tasks per node is unfavorable to the performance of global model. 
% This limit on training data overlap will hinder the performance of ring training topology especially when the number of nodes increase.

% \vspace{-3mm}
% \paragraph{\textbf{Mesh Topology}}

% , edge connections in Mesh topology are much denser, which is commonly seen in collaborative or \textit{ad-hoc} IoT clusters. 
	% Mesh topology's adjacent matrix $W$ can be generally formulated as:
% \scriptsize	
% \begin{equation}
% \begin{split}
% 	W_{i,j} = \left\{
% 	\begin{aligned}
% 		 C_{i,j}, &~~~~\text{If} ~~i \neq j;\\
% 		 0, &~~~~\text{Otherwise}.
% 	\end{aligned}
% 	\right.
% \end{split}
% \end{equation}
% \normalsize
% The matrix denotes that every node needs to broadcast its parameters to all other $n$-$1$ collaboration nodes except itself.	
% 	Clearly, this matrix is much denser than Ring matrix with all non-diagonal entries as non-zero elements. 

% In our collective learning system, Mesh topology represents the ideal case of collaboration with the most dense connection scenarios.
% 	This could bring great \textit{benefits in achieving global consensus} since every task components can be shared in multiple nodes.
% 	As we will show in later experiments, the Mesh topology always achieves the upper bound convergence performance. 
% 	However, Mesh topology can cause \textit{large communication overhead} especially in systems without efficient broadcasting mechanisms. 

% In real-world settings, the network topology often does not perfectly match Ring or Mesh, but lies in between, \textit{e.g.}, with communication connections with multiple neighbor nodes.
% 	Therefore, the convergence performance of these intermediate cases should be between the Ring (lower-bound) and Mesh (upper-bound) topologies.
% 	In the later sections, we will conduct experiments using both topologies to evaluate our collective learning system's generality.

% For our learning systems with Ring topology, our communication cost can be formulated as:
% \vspace{-1.5mm}
% \begin{small}
% \begin{equation}
% \scriptsize
% 	\medmuskip=-1mu
% 	\begin{aligned}
% 	 Q = N\sum_{i=1}^{L-D} B_w f_{i+1} (k_i)^{2} + P\sum_{i=D}^{L} B_w f_{i+1}F_{r}(k_i)^{2} 
% 	\end{aligned}
% 	\label{eq:comring}
% \vspace{-0.5mm}
% \end{equation}
% \end{small}

% 	In the real-world decentralized settings, network topologies vary a lot and thus the node collaborations can happen in many possible ways~\cite{x,x}. 
% 	As we know that, varied network topologies can incur different amounts of communication overheads.
% 	But on the other hand, such collaborative communication benefits the global consensus, therefore it brings better global model convergence performance.
% % Based on the model structure we proposed, the shared layers only account for a small portion of parameters. 
% % Thus, the communication for exchanging shared layers are ignored and the topology is discussed for exchanging task-specific modules.
% %collaborations between different local nodes are possible as long as they share partial training data. 
% %To optimize the performance on each global task, we suppose that all neural network \textbf{modules} trained for the same task will exchange their parameters. 
% %Thus, the allocation of training data over the decentralized system determines the relationships between different nodes in collaborative training. 
% Therefore, here we discuss two major topologies in large scale decentralized systems, namely Ring and Mesh~\cite{x,lee2006emerging}. 
% In our collaborative learning system, these two network topologies represent respectively the most harsh and mild conditions to fulfill our collaboration requirements.

==> _txt/8_impact.tex <==
\section{Broader Impact}
\label{sec:conc}
\vspace{-3mm}
By comprehensively integrating the proposed techniques to an innovative “Feature-Allocated Model Regulation” federated learning ramework, broad impacts will be brought into other scientific areas: (1) The enabled heterogeneous collaboration capability may support a much wider range of deep learning application with local tasks and Non-IID data constraints, such as spectrum monitoring in 5G wireless net-work and automatic public transportation system. (2) The optimized edge computation and communication may support more practical deployment on divergent edge devices with limited resources, such as smartphones and wearable devices. (3) Moreover, the scalable decentralized framework topology can also inspire further optimization and application exploration on intelligent IoT and edge computing systems. These research outcomes and application potentials will build a solid technical foundation for next-generation deep learning to support ubiquitous artificial intelligence applications.

